Near Optimal LP Rounding Algorithm for Correlation Clustering on Complete and Complete k-partite Graphs

We give new rounding schemes for the standard linear programming relaxation of the correlation clustering problem, achieving approximation factors almost matching the integrality gaps: - For complete graphs our appoximation is $2.06 - \varepsilon$ for a fixed constant $\varepsilon$, which almost matches the previously known integrality gap of $2$. - For complete $k$-partite graphs our approximation is $3$. We also show a matching integrality gap. - For complete graphs with edge weights satisfying triangle inequalities and probability constraints, our approximation is $1.5$, and we show an integrality gap of $1.2$. Our results improve a long line of work on approximation algorithms for correlation clustering in complete graphs, previously culminating in a ratio of $2.5$ for the complete case by Ailon, Charikar and Newman (JACM'08). In the weighted complete case satisfying triangle inequalities and probability constraints, the same authors give a $2$-approximation; for the bipartite case, Ailon, Avigdor-Elgrabli, Liberty and van Zuylen give a $4$-approximation (SICOMP'12).

==> files/k_partite_cases.tex <==
In this appendix, we bound the expected costs of the $6$ other triangles.  We
adopt the convention that the triangles have LP lengths $(a,b,c)$, with vertex
$u$ opposite edge $b$, vertex $v$ opposite edge $c$, and vertex $w$ opposite
edge $a$. Costs incurred when vertex $x \in \{u,v,w\}$ is a pivot will be enclosed in square brackets with subscript $x$, as in $[cost]_x$. Instead of writing, $ALG(uvw)$ and $LP(uvw)$,
we write $ALG$ and $LP$.

		\begin{center}
			\tikz\draw (1,1.3) node[above]{u} -- node[right]{a}
			(2,0) node[right]{v} -- node[below]{b}
			(0,0) node[left]{w} -- node[left]{c} (1,1.3);
		\end{center}

\medskip

\noindent\textbf{\ppp-Triangles:} If $a,b,c <\tfrac{1}{3}$ or $a,b,c \ge \tfrac{1}{3}$, then 
either no edges are cut and the algorithm makes no mistakes, or all edges are cut and
no edge is ever charged unsafely, so $ALG = 0$. The remaining cases are 
$a,b < \tfrac{1}{3} \le c$ and $a < \tfrac{1}{3} \le b,c$. In both cases,
			\begin{align*}
				ALG &= [f^+_3(c)(1-f^+_3(a)) + f^+_3(a)(1-f^+_3(c))]_u
					 + [f^+_3(a)(1-f^+_3(b)) + f^+_3(b)(1-f^+_3(a))]_v\\
					 &\qquad + [f^+_3(b)(1-f^+_3(c)) + f^+_3(c)(1-f^+_3(b))]_w,\\
				LP &= [b(1-f^+_3(c)f^+_3(a))]_u
					 + [c(1-f^+_3(a)f^+_3(b))]_v
					 + [a(1-f^+_3(b)f^+_3(c))]_w.
				\end{align*}
			When $a,b < \tfrac{1}{3} \le c$, $ALG = 2$, $LP = a+b+c \ge 2c \ge
			\tfrac{2}{3}$, where we apply the LP triangle inequality
			constraints. When $a < \tfrac{1}{3} \le b,c$, $ALG = 2$, $LP = c +
			b \ge \tfrac{2}{3}$. Therefore $3\cdot LP \ge ALG$ as desired.

\medskip

\noindent\textbf{\mmm-Triangles:} In this case, the function $f^-_3$ is the only one participating in the costs; the costs are
		\begin{align*}
			ALG &= [(1-f^-_3(a))(1-f^-_3(c))]_u + [(1-f^-_3(a))(1-f^-_3(b))]_v + [(1-f^-_3(c))(1-f^-_3(b))]_w\\
				&= 3 - 2a - 2b - 2c + ab + bc + ac,\\
			LP &= [(1-b)(1-f^-_3(a)f^-_3(c))]_u + [(1-c)(1-f^-_3(a)f^-_3(b))]_v + [(1-a)(1-f^-_3(c))f^-_3(b))]_w\\
			   &= 3 - a - b - c - ab - ac - bc + 3abc.
		\end{align*}
		We verify that the $3$-approximation holds:
		\begin{align*}
			3\cdot LP - ALG &= 6 - a - b - c - 4ab - 4ac - 4bc + 9abc \\
							&= 6 - a - b - 4ab - c(4a(1-b) + 4b(1-a) + (1 - ab))\\
							&\ge 5 - 5a - 5b + 5ab= 5(1-a)(1-b),
		\end{align*}
		where in the third inequality we have applied $c \le 1$. Thus, $3\cdot LP \ge ALG$ as desired.

\medskip

\noindent\textbf{\ppm-Triangles} Here, we must verify the cases $a,b < \tfrac{1}{3}$,
		$a < \tfrac{1}{3} \le b$, and $\tfrac{1}{3} \le a,b$. In all cases,
	\begin{align*}
		ALG &= [\fpk(a)(1-\fmk(c)) + \fmk(c)(1-\fpk(a))]_u
		+ [(1-\fpk(a))(1-\fpk(b))]_v
			\\&\qquad  + [f^+_3(b)(1-f^-_3(c)) + f^-_3(c)(1-f^+_3(b))]_w,\\
		LP &= [b(1 - \fpk(a)\fmk(c))]_u + [(1-c)(1-\fpk(a)\fpk(b))]_v + [a(1-\fpk(b)\fmk(c))]_w.
	\end{align*}
	When $a,b < \tfrac{1}{3}$, we have $ALG = 1 + 2c$, $LP = 1 - c + b + a\ge 1$, where we have applied the triangle inequality constraint to bound the LP. Since $c \le 1$, we have $3\cdot LP \ge ALG$.

	When $a < \tfrac{1}{3} \le b$, we have $ALG = 1$, $LP = 1 + a + b -c -ac\ge
	1 - ac \ge \frac{2}{3}$, where we have applied the triangle inequality
	constraint and the fact that $ac \le \tfrac{1}{3}$.

	When $\tfrac{1}{3} \le a,b$, we have $ALG = 2(1 -c)$, $LP = b(1-c) + a(1-c)
	\ge \tfrac{2}{3}(1-c)$, where we have applied the fact that $a+b \ge
	\tfrac{2}{3}$.  Thus, we have $3\cdot LP \ge ALG$ in this case as well.

\medskip

\noindent\textbf{\pmm-Triangles:} Here we must verify two cases: $a < \tfrac{1}{3}$ and $a \ge \tfrac{1}{3}$. In both cases, the costs are
	\begin{align*}
		ALG &= [(1-\fpk(a))(1-\fmk(c))]_u
		      + [(1-\fpk(a))(1-\fmk(b))]_v\\
			  &\qquad + [\fmk(c)(1-\fmk(b)) + \fmk(b)(1-\fmk(c))]_w,\\
		LP &= [(1-b)(1-\fpk(a)\fmk(c))]_u +[(1-c)(1-\fpk(a)\fmk(b))]_v + [a(1-\fmk(b)\fmk(c))]_w.
	\end{align*}
	When $a < \tfrac{1}{3}$, $ALG = 2 - 2bc$, $LP = 2 -b -c + a - abc$. We calculate,
	\begin{align*}
		3\cdot LP - ALG &= 4 - 3b - 3c + 3a + 2bc - 3abc 
		= 4(1-b)(1-c) + b + c - 2bc + 3a(1-bc)\\
		&= (1 - bc) + 3(1-b)(1-c) + 3a(1-bc)
		\ge 0,
	\end{align*}
	as desired.

	When $a \ge \tfrac{1}{3}$, $ALG = c + b -2bc$, $LP = 2 - 2b - 2c + 2bc + a(1-bc)$. Again we verify,
	\begin{align*}
		3\cdot LP - ALG &= 6 - 7b - 7c + 8bc + 3a(1-bc) \ge 7 - 7b - 7c + 7bc \\
			   &= 7(1-b)(1-c) \ge 0,
	\end{align*}
	where to get the inequality we applied the assumption $a \ge \frac{1}{3}$.

\medskip

\noindent\textbf{\ppn-Triangles:} Here, when $c \ge \tfrac{2}{3}$, the rounding is
	deterministic: if $a < \tfrac{1}{3} \le b$, $ALG = 1$, $LP = b \ge
	\tfrac{1}{3}$; if $\tfrac{1}{3} \le a,b$, the cost to the algorithm is
	zero. Crucially, it is not possible to have both $a,b < \tfrac{1}{3}$,
	because $a+b \ge c \ge \tfrac{2}{3}$.

	Now we deal with the cases where $c < \frac{2}{3}$. The costs are
	\begin{align*}
		ALG &= [\fnk(c)(1-\fpk(a)) + \fpk(a)(1-\fnk(c))]_u
			  +[\fnk(c)(1-\fpk(b)) + \fpk(b)(1-\fnk(c))]_w\\
		LP &=[b(1-\fnk(c)\fpk(a))]_u
			  +[a(1-\fnk(c)\fpk(b))]_w
	\end{align*}
	When $a,b < \tfrac{1}{3}$, $ALG = 3c$, and $LP = a+b \ge c$, where we applied the triangle inequality.

	When $a < \tfrac{1}{3} \le b$, we have $ALG = 1$, $LP = b + a(1-c) \ge \tfrac{1}{3}$, by our assumption on $b$.

	For $\tfrac{1}{3}\le a,b$, $ALG = 2(1-c)$ and $LP = (b+a)(1-c) \ge \tfrac{2}{3}(1-c)$. Therefore, $3\cdot LP \ge ALG$ holds in all cases.

\medskip

\noindent\textbf{\mmn-Triangles:}
		Here, when $c \ge \tfrac{2}{3}$, the algorithm never incurs cost on
		unsafe edges. Therefore, we must simply calculate the costs when
		$c < \tfrac{2}{3}$:
	\begin{align*}
		ALG &= [(1-\fnk(c))(1-\fmk(a))]_u
		+[(1-\fnk(c))(1-\fmk(b))]_w\\
		&= (1-\tfrac{3}{2}c)(2-a-b),\\
		LP &=[(1-b)(1-\fnk(c)\fmk(a))]_u
		+[(1-a)(1-\fnk(c)\fmk(b))]_w\\
		&= (1-b)(1-\tfrac{3}{2}ac) + (1-a)(1-\tfrac{3}{2}bc)
	\end{align*}
		We verify that $3\cdot LP \ge ALG$:
		\begin{align*}
			LP - ALG= 3c(1-b)(1-a)\ge 0.
		\end{align*}
		Thus the approximation holds.


	This concludes the case analysis for $k$-partite complete graphs.

